A comprehensive and FAIR comparison between MLP and KAN representations for differential equations and operator networks

Kolmogorov-Arnold Networks (KANs) were recently introduced as an alternative representation model to MLP. Herein, we employ KANs to construct physics-informed machine learning models (PIKANs) and deep operator models (DeepOKANs) for solving differential equations for forward and inverse problems. In particular, we compare them with physics-informed neural networks (PINNs) and deep operator networks (DeepONets), which are based on the standard MLP representation. We find that although the original KANs based on the B-splines parameterization lack accuracy and efficiency, modified versions based on low-order orthogonal polynomials have comparable performance to PINNs and DeepONet although they still lack robustness as they may diverge for different random seeds or higher order orthogonal polynomials. We visualize their corresponding loss landscapes and analyze their learning dynamics using information bottleneck theory. Our study follows the FAIR principles so that other researchers can use our benchmarks to further advance this emerging topic.

==> old_sec_nos.tex <==
\section{MLP and KAN in neural operators}
\label{Sec4}
In this section, we present comparative study of MLP and KAN in operator learning. We choose DeepONets as the representative neural operator. We note that in this section only Chebyshev KANs are employed.

\subsection{1D Burgers' equation}

\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
Model & $L^2$ relative error & No. of parameters & Time: ms/iter\\
\hline
DeepONet & $5.83\% \pm 0.19\%$ & 63900 & $1.9$ \\
DeepOKAN 1 & $2.71\% \pm 0.08\%$ & 252800 & $3.9$\\
DeepOKAN 2 & $3.02\%\pm 0.13\%$ & 76400 & $3.9$ \\
\hline
\end{tabular}
\caption{$L^2$ relative error of learning the solution operator of the 1D Burgers' equation with viscosity $\nu=\frac{1}{100\pi}$. The architectures are the branch and trunk nets are $[128, 100, 100, 100, 100]$ and $[4, 100, 100, 100]$, respectively, for DeepONet and DeepOKAN 1, and are $[128, 50, 50, 50, 50]$ and $[4, 50, 50, 50]$ for DeepOKAN 2. Here Chebyshev KAN is employed with degree three for both the branch and trunk nets.
}
\label{tab:burgers}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
Model & $1\%$ noise & $5\%$ noise & $10\%$ noise \\
\hline
DeepONet & $5.83\%\pm 0.19\%$ & $5.93\%\pm0.18\%$ & $6.29\%\pm0.19\%$\\
DeepOKAN 1 & $2.72\%\pm0.08\%$ & $2.94\%\pm0.09\%$ & $3.57\%\pm0.05\%$\\
DeepOKAN 2 & $3.02\%\pm0.13\%$ & $3.24\%\pm0.12\%$ & $3.91\%\pm0.13\%$ \\
\hline
\end{tabular}
\caption{TODO.
}
\label{tab:burgers2}
\end{table}

% \begin{table}[h]
% \centering
% \begin{tabular}{|c|c|c|c|c|}
% \hline
% & Model & $L^2$ relative error & No. of parameters & Time: ms/iter\\
% \hline
% $\nu=\frac{1}{10}$ & DeepONet & $2.09\% \pm 0.04\%$ & 63900 & $1.9$ \\

% & DeepOKAN 1 & $2.26\%\pm 0.05\%$ & 252800 & $3.9$\\
% & DeepOKAN 2 & $2.41\%\pm 0.06\%$ & 76400 &  $3.9$\\
% \hline
% $\nu=\frac{1}{100\pi}$ & DeepONet & $5.83\% \pm 0.19\%$ & 63900 & $1.9$ \\
% & DeepOKAN 1 & $2.71\% \pm 0.08\%$ & 252800 & $3.9$\\
% & DeepOKAN 2 & $3.02\%\pm 0.13\%$ & 76400 & $3.9$ \\
% \hline
% \end{tabular}
% \caption{$L^2$ relative error of learning the solution operator of the 1D Burgers' equation with viscosity $\nu=\frac{1}{10}$. The architectures are the branch and trunk nets are $[128, 100, 100, 100, 100]$ and $[4, 100, 100, 100]$, respectively, for DeepONet and DeepOKAN 1, and are $[128, 50, 50, 50, 50]$ and $[4, 50, 50, 50]$ for DeepOKAN 2. Here Chebyshev KAN is employed with degree three for both the branch and trunk nets.
% }
% \label{tab:burgers}
% \end{table}

% \begin{table}[h]
% \centering
% \begin{tabular}{|c|c|c|c|c|}
% \hline
% & Model & $1\%$ noise & $5\%$ noise & $10\%$ noise \\
% \hline
% $\nu=\frac{1}{10}$ & DeepONet & $2.14\% \pm 0.03\%$ & $3.04\%\pm 0.07\%$ & $4.83\%\pm0.06\%$\\
% & DeepOKAN 1 & $2.27\%\pm 0.05\%$ & $2.46\%\pm 0.06\%$ & $3.08\%\pm 0.04\%$\\
% & DeepOKAN 2 & $2.42\%\pm0.07\%$ & $2.64\%\pm0.05\%$ & $3.29\%\pm0.07\%$\\
% \hline
% $\nu=\frac{1}{100\pi}$ & DeepONet & $5.83\%\pm 0.19\%$ & $5.93\%\pm0.18\%$ & $6.29\%\pm0.19\%$\\
% & DeepOKAN 1 & $2.72\%\pm0.08\%$ & $2.94\%\pm0.09\%$ & $3.57\%\pm0.05\%$\\
% & DeepOKAN 2 & $3.02\%\pm0.13\%$ & $3.24\%\pm0.12\%$ & $3.91\%\pm0.13\%$ \\
% \hline
% \end{tabular}
% \caption{TODO.
% }
% \label{tab:burgers2}
% \end{table}

We consider the 1D Burgers equation with periodic boundary condition:
\begin{equation}
    \partial_tu + u\partial_x u = \nu \partial_{xx}u.
\end{equation}
where $\nu=\frac{1}{100\pi}$ denotes the viscosity. In this example, we learn the solution operator, which maps the initial condition, denoted as $u_0$, to the solution at $t=1$, using DeepONets and dataset from \cite{li2020fourier}. 
We apply four Fourier basis 
$$\{\cos(2\pi x), \sin(2\pi x), \cos(4\pi x), \sin(4\pi x)\}$$
to the input of the trunk net and data normalization to the output of DeepONets to improve the accuracy.
The errors are presented in Table \ref{tab:burgers}.

\subsection{120-dimensional Darcy problem}
In this section, we consider a 2D steady-state flow through porous media described by Darcy's law:
\begin{equation}
    \nabla\cdot(\lambda(x, y)\nabla u(x, y)) = f, x, y \in (0, 1),
\end{equation}
where $f = -30$ is a constant across field.
Here $\lambda$ denotes the hydraulic conductivity field and $u$ the hydraulic head. 
The boundary condition is specified as follows:
\begin{equation}
    u(0, y) = 1, u(1, y) = 0,
    \partial_{\mathbf{n}}u(x, 0) = \partial_{\mathbf{n}}u(x, 1) = 0.
\end{equation}
We learn the solution operator which maps $\log(\lambda)$ to $u$ using DeepONets and dataset from \cite{psaros2023uncertainty, zou2024neuraluq, zou2023uncertainty}. In this example, we normalize both the input and the output for better performance of DeepONets.

\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
 & $L^2$ relative error & No. of parameters & Time: ms/iter\\
\hline
DeepONet & $1.62\%\pm 0.15\%$ & 147000 & $2.3$ \\
\hline 
DeepOKAN & $2.18\%\pm0.02\%$ & 585200 & $8.8$ \\
\hline
\end{tabular}
\caption{Results for the Darcy problem, in which DeepONets (DeepONet and DeepOKAN) are employed to learn the solution operator.}
\label{tab:darcy}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
 & $1\%$ noise & $5\%$ noise & $10\%$ noise \\
\hline
DeepONet & $1.66\%\pm 0.15\%$ & $2.25\%\pm 0.12\%$ & $3.47\%\pm0.12\%$\\
\hline 
DeepOKAN & $2.18\%\pm0.02\%$ & $2.20\%\pm 0.02\%$ & $2.30\%\pm 0.03\%$\\
\hline
\end{tabular}
\caption{$L^2$ relative error for the Darcy problem
}
\label{tab:darcy2}
\end{table}

